Pilot Distributions for Phase Noise Estimation in Electro-Optic Frequency Comb Systems

We explore the optimal pilot positioning for phase tracking in electro-optic frequency comb setups. We show that, in contrast to previous results for regular multichannel systems, allocating the first and the last channels for pilots is optimal given a fixed pilot overhead

==> Figures/BER/ber_vs_M_2p.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

%
\definecolor{EKS_wd}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{RAT}{rgb}{0.85000,0.32500,0.09800}%
%\definecolor{EKS_dp}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{MS}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{WDT}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{EKS_dist}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{EKS_dp_subopt}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{UBE_dp_opt}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{UBE_dp_subopt}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{awgn}{rgb}{0.92900,0,0.92}%
% \pgfplotscreateplotcyclelist{list1}{%
% {color=ML_Demod,mark=triangle*,line width=\LineWidth pt},
% {color=Mcma,mark=+,line width=\LineWidth pt},
% {color=LS,mark=x,line width=\LineWidth pt},
% {color=LS_DDLMS,mark=star,line width=\LineWidth pt},
% {color=LS_Czegledi,mark=o,line width=\LineWidth pt},
% {color=LS_SW_Kabsch,mark=square,line width=\LineWidth pt},
% {color=SW_LS,mark=diamond,line width=\LineWidth pt},
% }
\newcommand\w{6.2}
\newcommand\h{3.3}
\newcommand\LineWidth{1}
\begin{tikzpicture}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0in,0in)},
scale only axis,
xmin=10,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={\scriptsize{ Number of Channels $L$}},
ymode=log,
ymin=0.0008,
ymax=0.03,
yminorticks=true,
xtick={20,40,60,80,100},
xticklabels={{$\text{20}$},{$\text{40}$},{$\text{60}$},{$\text{80}$},{$\text{100}$}},
ylabel style={font=\color{white!15!black}},
ylabel={\scriptsize{BER}},
ytick={0.001,0.01,0.1},
yticklabels={{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$}},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={BER plots when OHp = 0.01},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
grid style={dotted,white!70!black},
%legend style={legend cell align=left, align=left, draw=white!15!black}
legend style={at={(0.0,1)}, anchor=north west,font=\scriptsize,legend cell align=left, align=left},
%legend style={at={(0.0,1)}, anchor=north west,font=\scriptsize, fill=none,legend cell align=left, align=left, draw=none},
]
\pgfplotsset{every tick label/.append style={font=\scriptsize},}
% \addplot [color=red,line width=\LineWidth pt]
%   table[row sep=crcr]{%
% 10	0.00228608973168298\\
% 20	0.00163596934139965\\
% 30	0.00144589189569289\\
% 40	0.00143374880404323\\
% 50	0.00145070574750661\\
% 60	0.00146948938450575\\
% 70	0.00153797862797789\\
% 80	0.00167216464411846\\
% 90	0.00181250018756562\\
% 100	0.00201170647218185\\
% };
% \addlegendentry{UBE MS $\mathcal{D}=\{1,M\}$}

% \addplot [color=blue,line width=\LineWidth pt]
%   table[row sep=crcr]{%
% 10	0.0418181352781097\\
% 20	0.00469482712136038\\
% 30	0.00263505305560197\\
% 40	0.00218649625256928\\
% 50	0.00201605989672615\\
% 60	0.00184398586879364\\
% 70	0.00177861458194817\\
% 80	0.00193481994410549\\
% 90	0.00208049151605916\\
% 100	0.00236562996422052\\
% };
% \addlegendentry{UBE MS $\mathcal{D}=\{1,2\}$}



\addplot [color=MS,line width=\LineWidth pt, mark=triangle, mark options={solid, MS}]
  table[row sep=crcr]{%
10	0.00141936458180275\\
20	0.00129045248828763\\
30	0.00122361189139854\\
40	0.00120459191051662\\
50	0.00121022908358791\\
60	0.00112094002991362\\
70	0.00115319660216608\\
80	0.00112987521929102\\
90	0.00115053910047482\\
100	0.00119565037842019\\
};
\addlegendentry{\ac{RAT} $D =2$}
%\addlegendentry{\ac{RAT} $\mathcal{D}^{*}=\{1,M\}$}
%-------------------------------------
% RAT D3
%-------------------------------------
%  \addplot [color=MS,line width=\LineWidth pt,dashed, mark=otimes*, mark options={solid,ForestGreen}]
%   table[row sep=crcr]{%
% 10	0.00143433032385866\\
% 20	0.00130374521463342\\
% 30	0.00125836690981413\\
% 40	0.00118980526372379\\
% 50	0.0012607565122082\\
% 60	0.0011724049806661\\
% 70	0.00115764151133557\\
% 80	0.00114733145728718\\
% 90	0.00112928585462066\\
% 100	0.0011333677908556\\
% };
% \addlegendentry{\ac{RAT} $D =3$}
%---------------------------------------------
%RAT D = L+1/2
%------------------------------------------------

\addplot [color=MS,line width=\LineWidth pt, mark=o, mark options={solid, ForestGreen}]
  table[row sep=crcr]{%
10	0.00150134522436846\\
20	0.0015123995333381\\
30	0.0014915947569696\\
40	0.00154318153216124\\
50	0.00164565264922382\\
60	0.001568155868134\\
70	0.001622469554836\\
80	0.00171270315574667\\
90	0.00177991562001474\\
100	0.00186235211233389\\
};
\addlegendentry{\ac{RAT} $D = (L+1)/2 $}
%\addlegendentry{\ac{RAT} $\mathcal{D}^{*}=\{1,2,\dots,\lfloor M/2\rfloor\}$}

\addplot [color=MS,line width=\LineWidth pt, mark=asterisk, mark options={solid, Red}]
  table[row sep=crcr]{%
10	0.00191292517006803\\
20	0.0020108843537415\\
30	0.00203185941043084\\
40	0.00204345238095238\\
50	0.0020131195335277\\
60	0.00245221898283123\\
70	0.00228585311675691\\
80	0.00251123663751215\\
90	0.00270678112514847\\
100	0.00292298347910593\\
};
\addlegendentry{\ac{RAT} $D =L$}
%\addlegendentry{\ac{RAT} $\mathcal{D}=\{1,2,\dots,M\}$}

\addplot [color=WDT,line width=\LineWidth pt,densely dashed, mark=square, mark options={solid, WDT}]
  table[row sep=crcr]{%
10	0.00144725232937898\\
20	0.00128527409893209\\
30	0.00123434312922937\\
40	0.00127228224666276\\
50	0.00137201002383527\\
60	0.00157644953061588\\
70	0.0019355412994831\\
80	0.00280912250630862\\
90	0.00835996141803177\\
100	0.0152003297268259\\
};
\addlegendentry{\ac{WDT}}

% \addplot [color=ForestGreen,solid,line width=\LineWidth pt]
%   table[row sep=crcr]{%
% 10	0.00101909522857689\\
% 20	0.00101909522857689\\
% 30	0.00101909522857689\\
% 40	0.00101909522857689\\
% 50	0.00101909522857689\\
% 60	0.00101909522857689\\
% 70	0.00101909522857689\\
% 80	0.00101909522857689\\
% 90	0.00101909522857689\\
% 100	0.00101909522857689\\
% };
% \addlegendentry{AWGN}

\end{axis}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%

==> Figures/SOP_Results/Pol_tolerance_fixed_mu.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.534in,
at={(0.758in,0.513in)},
scale only axis,
xmode=log,
xmin=1e-08,
xmax=0.001,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$\Delta_p\times T$},
ymode=log,
ymin=0.0001,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
title={16-QAM SER  $\eta$ = 18.28 dB},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00114481289625792\\
1e-07	0.00114527290545811\\
3.57142857142857e-07	0.00114559791195824\\
1e-06	0.00114495289905798\\
3.57142857142857e-06	0.00114561791235825\\
1e-05	0.00114503790075801\\
3.57142857142857e-05	0.00114555291105822\\
6.07142857142857e-05	0.00114584791695834\\
0.0001	0.00114514290285806\\
0.000178571428571429	0.00114493789875797\\
0.000357142857142857	0.00114583291665833\\
0.001	0.00114531790635813\\
};
\addlegendentry{AWGN}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00165279048490393\\
1e-07	0.00180721930253835\\
3.57142857142857e-07	0.00233057086320986\\
1e-06	0.00416183323049427\\
3.57142857142857e-06	0.0214221472797293\\
1e-05	0.122039069980212\\
3.57142857142857e-05	0.69367265260963\\
6.07142857142857e-05	0.792566762058767\\
0.0001	0.830544947764846\\
0.000178571428571429	0.849878151662801\\
0.000357142857142857	0.860237276325028\\
0.001	0.867360443839231\\
};
\addlegendentry{MCMA}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.0011847539309347\\
1e-07	0.00122301538330603\\
3.57142857142857e-07	0.00133168790825337\\
1e-06	0.00165258835294368\\
3.57142857142857e-06	0.00362984850741505\\
1e-05	0.0185478786782698\\
3.57142857142857e-05	0.703411907700164\\
6.07142857142857e-05	0.800206701206409\\
0.0001	0.829832975169684\\
0.000178571428571429	0.844712126853763\\
0.000357142857142857	0.85254226153748\\
0.001	0.858838985935871\\
};
\addlegendentry{UDDLMS}

\addplot [color=mycolor4, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00118476456945892\\
1e-07	0.00122301538330603\\
3.57142857142857e-07	0.00133168790825337\\
1e-06	0.0016525989914679\\
3.57142857142857e-06	0.00362984850741505\\
1e-05	0.0185478786782698\\
3.57142857142857e-05	0.703349603183047\\
6.07142857142857e-05	0.800029596374391\\
0.0001	0.829745058405498\\
0.000178571428571429	0.844806256516096\\
0.000357142857142857	0.852598374433498\\
0.001	0.858890811506628\\
};
\addlegendentry{Czegledi}

\addplot [color=mycolor5, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00134876273963276\\
1e-07	0.00135244366901423\\
3.57142857142857e-07	0.00135818847209515\\
1e-06	0.00138036447583991\\
3.57142857142857e-06	0.00147356326730356\\
1e-05	0.00171862699206366\\
3.57142857142857e-05	0.00304744249877657\\
6.07142857142857e-05	0.00549029766590779\\
0.0001	0.0677201589395519\\
0.000178571428571429	0.426594991382795\\
0.000357142857142857	0.688957669312113\\
0.001	0.819829969786591\\
};
\addlegendentry{SW-Kabsch}

\addplot [color=mycolor6, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00223778165492883\\
1e-07	0.00225089363603481\\
3.57142857142857e-07	0.00227948466988659\\
1e-06	0.00235626289921062\\
3.57142857142857e-06	0.00265142343454116\\
1e-05	0.0035818794016894\\
3.57142857142857e-05	0.0100348677631439\\
6.07142857142857e-05	0.0243264165195004\\
0.0001	0.19106110236388\\
0.000178571428571429	0.569527708036341\\
0.000357142857142857	0.77941771633439\\
0.001	0.846596310559799\\
};
\addlegendentry{Louchet}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%

==> Figures/SOP_Results/SER_vs_SOP.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{AWGN}{rgb}{0.00000,0,0}%
\definecolor{MCMA}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{UDDLMS}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{Czegledi}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{SW-Kabsch}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{Louchet}{rgb}{0.30100,0.74500,0.93300}%
%
% \definecolor{SW_LS}{rgb}{0.85000,0.32500,0.09800}%
% \definecolor{LS}{rgb}{0.00000,0.44700,0.74100}%
% \definecolor{LS_DDLMS}{rgb}{0.63500,0.07800,0.18400}%
% \definecolor{LS_Czegledi}{rgb}{0.30100,0.74500,0.93300}%
% \definecolor{Mcma}{rgb}{0.49400,0.18400,0.55600}%
% \definecolor{LS_SW_Kabsch}{rgb}{0.92900,0.69400,0.12500}%
% \definecolor{ML_Demod}{rgb}{0.92900,0,0.92}%
%
\newcommand\w{7}
\newcommand\h{5}
\newcommand\LineWidth{1.1}


\pgfplotscreateplotcyclelist{list1}{%
{color=AWGN,mark=triangle*,line width=\LineWidth pt},
{color=MCMA,mark=oplus,mark size=2.5pt,mark options=solid,line width=\LineWidth pt,densely dotted},
{color=MCMA,mark=oplus*,mark size=2.5pt,mark options=solid,line width=\LineWidth pt, densely dashed},
%{color=LS,mark=x,line width=\LineWidth pt},
{color=Louchet,mark=x,,mark size=2.5pt,mark options=solid,line width=\LineWidth pt,densely dashed},
{color=Czegledi,mark=square,,mark options=solid,line width=\LineWidth pt,densely dotted},
{color=Czegledi,mark=square*,,mark size=2.5pt,mark options=solid,mark size=2pt,line width=\LineWidth pt,densely dashed},
{color=SW-Kabsch,mark=triangle,mark size=2.5pt,mark options=solid,line width=\LineWidth pt,densely dashed}
}

\begin{tikzpicture}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0cm,0cm)},
scale only axis,
xmode=log,
xmin=1e-08,
xmax=0.001,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$\Deltaptot\cdot T$},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER  $\eta$ = 18 dB},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
grid style={dotted,white!70!black},
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black}
]
\pgfplotsset{cycle list name=list1}

\addplot %[color=AWGN, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00116139984130859\\
1e-07	0.00116114044189453\\
3.57142857142857e-07	0.00116139221191406\\
1e-06	0.00116106414794922\\
3.57142857142857e-06	0.00116110992431641\\
1e-05	0.00116070556640625\\
3.57142857142857e-05	0.0011612548828125\\
6.07142857142857e-05	0.00116164398193359\\
0.0001	0.00116092681884766\\
0.000178571428571429	0.00116120910644531\\
0.000357142857142857	0.00116099548339844\\
0.001	0.00116210174560547\\
};
\addlegendentry{AWGN ($\Hb$ is known)}

\addplot %[color=MCMA, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00165279048490393\\
1e-07	0.00180721930253835\\
3.57142857142857e-07	0.00233057086320986\\
1e-06	0.00416183323049427\\
3.57142857142857e-06	0.0214221472797293\\
1e-05	0.122039069980212\\
3.57142857142857e-05	0.69367265260963\\
6.07142857142857e-05	0.792566762058767\\
0.0001	0.830544947764846\\
0.000178571428571429	0.849878151662801\\
0.000357142857142857	0.860237276325028\\
0.001	0.867360443839231\\
};
\addlegendentry{MCMA $\smash{\mu= 10^{-3}}$}

\addplot %[color=MCMA, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00141986461478523\\
1e-07	0.00181232752183371\\
3.57142857142857e-07	0.00232188889971105\\
1e-06	0.00344746112139216\\
3.57142857142857e-06	0.00727839193532677\\
1e-05	0.0225552822960294\\
3.57142857142857e-05	0.0606591669101652\\
6.07142857142857e-05	0.108133964806337\\
0.0001	0.227371960325963\\
0.000178571428571429	0.482493360605175\\
0.000357142857142857	0.706620799649362\\
0.001	0.822459920132463\\
};
\addlegendentry{MCMA opt. $\mu$}

% \addplot %[color=UDDLMS, line width=2.0pt]
%   table[row sep=crcr]{%
% 1e-08	0.00124018700691536\\
% 1e-07	0.00125943962858349\\
% 3.57142857142857e-07	0.00131039576637122\\
% 1e-06	0.00143156878023441\\
% 3.57142857142857e-06	0.00189876140385052\\
% 1e-05	0.00241665855004708\\
% 3.57142857142857e-05	0.0036831596376741\\
% 6.07142857142857e-05	0.00425004869971754\\
% 0.0001	0.0187834567059511\\
% 0.000178571428571429	0.184101774293042\\
% 0.000357142857142857	0.468560663614818\\
% 0.001	0.714877812408688\\
% };
% \addlegendentry{UDDLMS}
\addplot %[color=Louchet, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00162006915359891\\
1e-07	0.00162741469432811\\
3.57142857142857e-07	0.00164837180611019\\
1e-06	0.00177679296126749\\
3.57142857142857e-06	0.00230447063407032\\
1e-05	0.00428927632219733\\
3.57142857142857e-05	0.0248860832440505\\
6.07142857142857e-05	0.149208069543197\\
0.0001	0.553496461153859\\
0.000178571428571429	0.763931812278822\\
0.000357142857142857	0.83112380279861\\
0.001	0.855146293951495\\
};
\addlegendentry{\ac{DD-Kabsch}}

\addplot %[color=Czegledi, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00118476456945892\\
1e-07	0.00122301538330603\\
3.57142857142857e-07	0.00133168790825337\\
1e-06	0.0016525989914679\\
3.57142857142857e-06	0.00362984850741505\\
1e-05	0.0185478786782698\\
3.57142857142857e-05	0.703349603183047\\
6.07142857142857e-05	0.800029596374391\\
0.0001	0.829745058405498\\
0.000178571428571429	0.844806256516096\\
0.000357142857142857	0.852598374433498\\
0.001	0.858890811506628\\
};
\addlegendentry{\ac{DD-Czegledi} $\smash{\mu=10^{-3}}$}

\addplot %[color=Czegledi, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00118537547482225\\
1e-07	0.00122474107983507\\
3.57142857142857e-07	0.00129628908152333\\
1e-06	0.00141086328365962\\
3.57142857142857e-06	0.00171039901301906\\
1e-05	0.002240649654232\\
3.57142857142857e-05	0.00498658322781728\\
6.07142857142857e-05	0.0109313009317879\\
0.0001	0.0445932112593747\\
0.000178571428571429	0.268354071296386\\
0.000357142857142857	0.527018725041395\\
0.001	0.771657503003149\\
};
\addlegendentry{\ac{DD-Czegledi} opt. $\mu$}

\addplot %[color=SW-Kabsch, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00135058114996266\\
1e-07	0.00135571085354372\\
3.57142857142857e-07	0.00136138437063732\\
1e-06	0.00138498750040583\\
3.57142857142857e-06	0.00147836920879192\\
1e-05	0.00172030940553878\\
3.57142857142857e-05	0.0030423038213045\\
6.07142857142857e-05	0.00600539755202753\\
0.0001	0.0433418720171423\\
0.000178571428571429	0.407241250284082\\
0.000357142857142857	0.682731348008181\\
0.001	0.818800688289341\\
};
\addlegendentry{SW-Kabsch}



\end{axis}
\end{tikzpicture}%

==> Figures/SOP_Results/SER_vs_SOP_fixed_mu.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{AWGN}{rgb}{0.00000,0,0}%
\definecolor{MCMA}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{UDDLMS}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{Czegledi}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{SW-Kabsch}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{Louchet}{rgb}{0.30100,0.74500,0.93300}%
%
% \definecolor{SW_LS}{rgb}{0.85000,0.32500,0.09800}%
% \definecolor{LS}{rgb}{0.00000,0.44700,0.74100}%
% \definecolor{LS_DDLMS}{rgb}{0.63500,0.07800,0.18400}%
% \definecolor{LS_Czegledi}{rgb}{0.30100,0.74500,0.93300}%
% \definecolor{Mcma}{rgb}{0.49400,0.18400,0.55600}%
% \definecolor{LS_SW_Kabsch}{rgb}{0.92900,0.69400,0.12500}%
% \definecolor{ML_Demod}{rgb}{0.92900,0,0.92}%
%
\newcommand\w{7}
\newcommand\h{5}
\newcommand\LineWidth{1.2}


\pgfplotscreateplotcyclelist{list1}{%
{color=AWGN,mark=triangle*,line width=\LineWidth pt},
{color=MCMA,mark=+,mark options=solid,line width=\LineWidth pt,densely dashed},
%{color=LS,mark=x,line width=\LineWidth pt},
{color=Louchet,mark=square,mark options=solid,line width=\LineWidth pt,densely dashed},
{color=Czegledi,mark=star,mark options=solid,line width=\LineWidth pt,densely dashed},
{color=SW-Kabsch,mark=o,mark options=solid,line width=\LineWidth pt,densely dashed}
}

\begin{tikzpicture}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0cm,0cm)},
scale only axis,
xmode=log,
xmin=1e-08,
xmax=0.001,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$\Delta_{p_{tot}}\cdot T$},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER  $\eta$ = 18 dB},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
grid style={dotted,white!70!black},
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\pgfplotsset{cycle list name=list1}

\addplot %[color=AWGN, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00116139984130859\\
1e-07	0.00116114044189453\\
3.57142857142857e-07	0.00116139221191406\\
1e-06	0.00116106414794922\\
3.57142857142857e-06	0.00116110992431641\\
1e-05	0.00116070556640625\\
3.57142857142857e-05	0.0011612548828125\\
6.07142857142857e-05	0.00116164398193359\\
0.0001	0.00116092681884766\\
0.000178571428571429	0.00116120910644531\\
0.000357142857142857	0.00116099548339844\\
0.001	0.00116210174560547\\
};
\addlegendentry{$\Hb$ is known}

\addplot %[color=MCMA, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00165279048490393\\
1e-07	0.00180721930253835\\
3.57142857142857e-07	0.00233057086320986\\
1e-06	0.00416183323049427\\
3.57142857142857e-06	0.0214221472797293\\
1e-05	0.122039069980212\\
3.57142857142857e-05	0.69367265260963\\
6.07142857142857e-05	0.792566762058767\\
0.0001	0.830544947764846\\
0.000178571428571429	0.849878151662801\\
0.000357142857142857	0.860237276325028\\
0.001	0.867360443839231\\
};
\addlegendentry{MCMA}

% \addplot %[color=UDDLMS, line width=2.0pt]
%   table[row sep=crcr]{%
% 1e-08	0.00124018700691536\\
% 1e-07	0.00125943962858349\\
% 3.57142857142857e-07	0.00131039576637122\\
% 1e-06	0.00143156878023441\\
% 3.57142857142857e-06	0.00189876140385052\\
% 1e-05	0.00241665855004708\\
% 3.57142857142857e-05	0.0036831596376741\\
% 6.07142857142857e-05	0.00425004869971754\\
% 0.0001	0.0187834567059511\\
% 0.000178571428571429	0.184101774293042\\
% 0.000357142857142857	0.468560663614818\\
% 0.001	0.714877812408688\\
% };
% \addlegendentry{UDDLMS}
\addplot %[color=Louchet, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.0011847539309347\\
1e-07	0.00122301538330603\\
3.57142857142857e-07	0.00133168790825337\\
1e-06	0.00165258835294368\\
3.57142857142857e-06	0.00362984850741505\\
1e-05	0.0185478786782698\\
3.57142857142857e-05	0.703411907700164\\
6.07142857142857e-05	0.800206701206409\\
0.0001	0.829832975169684\\
0.000178571428571429	0.844712126853763\\
0.000357142857142857	0.85254226153748\\
0.001	0.858838985935871\\
};
\addlegendentry{Kabsch}

\addplot %[color=Czegledi, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00118476456945892\\
1e-07	0.00122301538330603\\
3.57142857142857e-07	0.00133168790825337\\
1e-06	0.0016525989914679\\
3.57142857142857e-06	0.00362984850741505\\
1e-05	0.0185478786782698\\
3.57142857142857e-05	0.703349603183047\\
6.07142857142857e-05	0.800029596374391\\
0.0001	0.829745058405498\\
0.000178571428571429	0.844806256516096\\
0.000357142857142857	0.852598374433498\\
0.001	0.858890811506628\\
};
\addlegendentry{Czegledi}

\addplot %[color=SW-Kabsch, line width=2.0pt]
  table[row sep=crcr]{%
1e-08	0.00134876273963276\\
1e-07	0.00135244366901423\\
3.57142857142857e-07	0.00135818847209515\\
1e-06	0.00138036447583991\\
3.57142857142857e-06	0.00147356326730356\\
1e-05	0.00171862699206366\\
3.57142857142857e-05	0.00304744249877657\\
6.07142857142857e-05	0.00549029766590779\\
0.0001	0.0677201589395519\\
0.000178571428571429	0.426594991382795\\
0.000357142857142857	0.688957669312113\\
0.001	0.819829969786591\\
};
\addlegendentry{SW-Kabsch}



\end{axis}
\end{tikzpicture}%

==> Figures/SOP_Results/SOP_SER_vs_SNR.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{AWGN}{rgb}{0.00000,0,0}%
\definecolor{MCMA}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{UDDLMS}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{Czegledi}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{SW-Kabsch}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{Louchet}{rgb}{0.30100,0.74500,0.93300}%
%
% \definecolor{SW_LS}{rgb}{0.85000,0.32500,0.09800}%
% \definecolor{LS}{rgb}{0.00000,0.44700,0.74100}%
% \definecolor{LS_DDLMS}{rgb}{0.63500,0.07800,0.18400}%
% \definecolor{LS_Czegledi}{rgb}{0.30100,0.74500,0.93300}%
% \definecolor{Mcma}{rgb}{0.49400,0.18400,0.55600}%
% \definecolor{LS_SW_Kabsch}{rgb}{0.92900,0.69400,0.12500}%
% \definecolor{ML_Demod}{rgb}{0.92900,0,0.92}%
%
\newcommand\w{5}
\newcommand\h{4}
\newcommand\LineWidth{1.5}

\newcommand\xMax{20}
\newcommand\xMin{14}
\newcommand\yMax{1}

\pgfplotscreateplotcyclelist{list1}{%
{color=AWGN,mark=triangle*,mark options=solid,line width=\LineWidth pt},
{color=MCMA,mark=+,mark options=solid,line width=\LineWidth pt,densely dashed},
%{color=LS,mark=x,line width=\LineWidth pt},
{color=Louchet,mark=square,mark options=solid,line width=\LineWidth pt,densely dashed},
{color=Czegledi,mark=star,mark options=solid,line width=\LineWidth pt,densely dashed},
{color=SW-Kabsch,mark=o,mark options=solid,line width=\LineWidth pt,densely dashed}
}

\begin{tikzpicture}

\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0*\w cm,0*\w cm)},
scale only axis,
xmin=\xMin,
xmax=\xMax,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
%tick label style={font =\thin},
xticklabels={$\text{13}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black},
legend style={at={(0.1,1.1)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
legend columns=5
]

\pgfplotsset{cycle list name=list1}
%+++++++++++ AWGN+++++++++++ 
\addplot %[color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
12	0.20400341796875\\
13	0.129314956665039\\
14	0.0726002578735352\\
15	0.0351884613037109\\
16	0.014272819519043\\
17	0.00464485931396484\\
18	0.00116139984130859\\
19	0.000215545654296875\\
20	3.65753173828125e-05\\
21	1.60369873046875e-05\\
22	1.45111083984375e-05\\
};
\addlegendentry{AWGN ($\Hb$ is known)}

%+++++++++++ MCMA +++++++++++ 
\addplot %[color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
12	0.226635271582091\\
13	0.14468264017402\\
14	0.0823198759780527\\
15	0.0403916187786111\\
16	0.0166090305509561\\
17	0.00553118405246583\\
18	0.00141986461478523\\
19	0.000264155384565437\\
20	4.77257231908056e-05\\
21	2.27265348527645e-06\\
22	4.44790753546963e-05\\
};
\addlegendentry{MCMA \cite{oh_MCMA:1995}}

%+++++++++++ UDDLMS +++++++++++ 
% \addplot %[color=mycolor3, line width=2.0pt]
%   table[row sep=crcr]{%
% 12	0.207613640790883\\
% 13	0.132046078049414\\
% 14	0.0745016395571572\\
% 15	0.0363553780721405\\
% 16	0.0148592253498263\\
% 17	0.00491150449660725\\
% 18	0.00124018700691536\\
% 19	0.000225463458978605\\
% 20	2.71257426706925e-05\\
% 21	1.67202363559625e-06\\
% 22	8.11661959027304e-08\\
% };
% \addlegendentry{UDDLMS}

%+++++++++++ Louchet +++++++++++ 
\addplot %[color=mycolor6, line width=2.0pt]
  table[row sep=crcr]{%
12	0.224926796207915\\
13	0.145109379565598\\
14	0.0834432729456836\\
15	0.0417307717281906\\
16	0.0175860767507549\\
17	0.00602338398103958\\
18	0.00162006915359891\\
19	0.000492102529138665\\
20	0.000164353430083439\\
21	4.15083925846563e-05\\
22	1.15083925846563e-05\\
};
\addlegendentry{\ac{DD-Kabsch}\cite{Louchet:2014}}

%+++++++++++ Czegledi +++++++++++ 
\addplot %[color=mycolor4, line width=2.0pt]
  table[row sep=crcr]{%
12	0.206683622284991\\
13	0.131233661244765\\
14	0.0738241290867179\\
15	0.0358561735008604\\
16	0.0151569835394955\\
17	0.0047626862764196\\
18	0.00118537547482225\\
19	0.000211072692445051\\
20	2.41063601831109e-05\\
21	1.47722476542969e-06\\
22	1.13632674263823e-07\\
};
\addlegendentry{\ac{DD-Czegledi}\cite{Czegledi:2016}}

%+++++++++++ SW-Kabsch +++++++++++ 
\addplot %[color=mycolor5, line width=2.0pt]
  table[row sep=crcr]{%
12	0.225414166747833\\
13	0.142929620791533\\
14	0.0804707314697575\\
15	0.0392832537904613\\
16	0.0160782929125678\\
17	0.00532446186812116\\
18	0.00135058114996266\\
19	0.000246842634979384\\
20	2.99016265705659e-05\\
21	1.80188954904061e-06\\
22	9.73994350832765e-08\\
};
\addlegendentry{SW-Kabsch}


\end{axis}
%=================================================================
%                   Figure 2 Deltap_T = 1 e-6
%=================================================================
% \begin{axis}[%
% width=\w cm,
% height=\h cm,
% at={(6cm,0cm)},
% scale only axis,
% xmin = \xMin=12,
% xmax=\xMax,
% xlabel style={font=\color{white!15!black}},
% xlabel={$\text{SNR}$ (dB)},
% ymode=log,
% ymin=0.001,
% ymax = \yMax=1,
% yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
% xticklabels={$\text{13}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
% yminorticks=true,
% ylabel style={font=\color{white!15!black}},
% %ylabel={SER},
% axis background/.style={fill=white},
% title style={font=\bfseries},
% %title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
% xmajorgrids,
% ymajorgrids,
% yminorgrids,
% axis background/.style={fill=white},
% axis x line*=bottom,
% axis y line*=left,
% grid style={dotted,white!70!black}
% ]
% \pgfplotsset{cycle list name=list1}
% %+++++++++++ AWGN+++++++++++ 
% \addplot %[color=ML_Demod, line width=1.0pt, mark=*]
%   table[row sep=crcr]{%
% 12	0.203995956420898\\
% 13	0.129312828063965\\
% 14	0.0725890197753906\\
% 15	0.0351843795776367\\
% 16	0.0142663269042969\\
% 17	0.00464344024658203\\
% 18	0.00116106414794922\\
% 19	0.000215476989746094\\
% 20	3.66592407226562e-05\\
% 21	1.6082763671875e-05\\
% 22	1.4495849609375e-05\\
% };

% %+++++++++++  MCMA+++++++++++ 
% \addplot %[color=Mcma, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.251058358494854\\
% 13	0.167486875426123\\
% 14	0.100821588584786\\
% 15	0.0539323479757151\\
% 16	0.0251784357650726\\
% 17	0.010106952696341\\
% 18	0.00344746112139216\\
% 19	0.000986153046978995\\
% 20	0.000241014902113568\\
% 21	5.13863186260186e-05\\
% 22	1.03324567384176e-05\\
% };
% %\addlegendentry{MCMA}
% %+++++++++++  UDDLMS+++++++++++ 
% % \addplot %[color=LS, line width=1.0pt]
% %   table[row sep=crcr]{%
% % 12	0.216066182916139\\
% % 13	0.138072960293497\\
% % 14	0.0783778448751664\\
% % 15	0.0385969449043862\\
% % 16	0.0159969319177949\\
% % 17	0.00538445180351287\\
% % 18	0.00141086328365962\\
% % 19	0.00027109509431512\\
% % 20	3.57780591539236e-05\\
% % 21	2.8895165741372e-06\\
% % 22	1.29865913444369e-07\\
% % };
% % %\addlegendentry{UDDLMS}
% %+++++++++++  Louchet+++++++++++ 
% \addplot %[color=LS_DDLMS, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.227444108957502\\
% 13	0.147282774909906\\
% 14	0.0851328771793124\\
% 15	0.042989837992273\\
% 16	0.0183534950163956\\
% 17	0.00642382552514529\\
% 18	0.00177679296126749\\
% 19	0.000421845069965261\\
% 20	0.000164353430083439\\
% 21	4.15083925846563e-05\\
% 22	1.15083925846563e-05\\
% };

%% +++++++++++ Czegledi+++++++++++ 
% \addplot %[color=LS_Czegledi, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.226052157397487\\
% 13	0.143448418882504\\
% 14	0.080885815395604\\
% 15	0.0395526443946625\\
% 16	0.016229951949612\\
% 17	0.00540018181227882\\
% 18	0.00138498750040583\\
% 19	0.000257085808902309\\
% 20	3.28073763838836e-05\\
% 21	2.32135320281809e-06\\
% 22	1.29865913444369e-07\\
% };
%% +++++++++++ SW-Kabsch+++++++++++ 

% \addplot %[color=LS_SW_Kabsch, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.227444108957502\\
% 13	0.147282774909906\\
% 14	0.0851328771793124\\
% 15	0.042989837992273\\
% 16	0.0183534950163956\\
% 17	0.00642382552514529\\
% 18	0.00177679296126749\\
% 19	0.000421845069965261\\
% 20	0.000164353430083439\\
% 21	4.15083925846563e-05\\
% 22	1.15083925846563e-05\\
% };
% %\addlegendentry{SW-Kabsch}

% \end{axis}
%=================================================================
%                   Figure 2 Deltap_T = 3.57 e-6
%=================================================================
%-************
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(\w cm+1cm,0cm)},
scale only axis,
xmin =\xMin,
xmax=\xMax,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax=1,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
xticklabels={$\text{13}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\color{white!15!black}},
%ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black}
]
%+++++++ AWGN +++++++++
\pgfplotsset{cycle list name=list1}
\addplot %AWGN
  table[row sep=crcr]{%
12	0.203999794006348\\
13	0.129312927246094\\
14	0.0725995941162109\\
15	0.0351876449584961\\
16	0.0142747344970703\\
17	0.00464553070068359\\
18	0.0011612548828125\\
19	0.000215400695800781\\
20	3.66744995117188e-05\\
21	1.60446166992188e-05\\
22	1.45034790039063e-05\\
};

%+++++++ MCMA +++++++++
\addplot %MCMA
  table[row sep=crcr]{%
12	0.272158436414402\\
13	0.188032101230479\\
14	0.119150368494529\\
15	0.0686895230674329\\
16	0.0358239018213694\\
17	0.0168980633745658\\
18	0.00727839193532677\\
19	0.00293043245349177\\
20	0.00114109119833772\\
21	0.000452469075679362\\
22	0.000190326612772313\\
};

%+++++++ Louchet +++++++++
\addplot %Louchet
  table[row sep=crcr]{%
12	0.234100378234473\\
13	0.15308102009675\\
14	0.0898410684718029\\
15	0.0464115856628032\\
16	0.0205804357001396\\
17	0.00763803934937177\\
18	0.00230447063407032\\
19	0.000548926982890166\\
20	0.000139605856952697\\
21	0.000164353430083439\\
22	4.15083925846563e-05\\
};

%+++++++ UDDLMS +++++++++
% \addplot %
%   table[row sep=crcr]{%
% 12	0.230185294308626\\
% 13	0.148997832862569\\
% 14	0.0862149280867504\\
% 15	0.0436257345540729\\
% 16	0.0188057205934872\\
% 17	0.00671083731047693\\
% 18	0.00189876140385052\\
% 19	0.000409662023960261\\
% 20	6.17187753644362e-05\\
% 21	6.34719651959352e-06\\
% 22	3.7336450115256e-07\\
% };

%+++++++ Czegledi +++++++++
\addplot %Czegledi
  table[row sep=crcr]{%
12	0.229022523619363\\
13	0.147398079607805\\
14	0.0845530421090224\\
15	0.0422491315217038\\
16	0.0178888510113308\\
17	0.00622526866010844\\
18	0.00171039901301906\\
19	0.00034868186097854\\
20	5.0891204831012e-05\\
21	4.80503879744164e-06\\
22	2.92198305249829e-07\\
};

%+++++++SW-Kabsch+++++++++

\addplot %SW-Kabsch
  table[row sep=crcr]{%
12	0.227776208564657\\
13	0.144794990422389\\
14	0.0819214473556053\\
15	0.0402807132885296\\
16	0.0167021606441349\\
17	0.0056336807246518\\
18	0.00147836920879192\\
19	0.000281938898087725\\
20	3.66871205480341e-05\\
21	2.85705009577611e-06\\
22	1.46099152624915e-07\\
};
\end{axis}
%*************

%=================================================================
%                   Figure 3 DeltaP_T 3.57e-5
%=================================================================
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(2*\w cm+2cm,0cm)},
scale only axis,
xmin = \xMin=12,
xmax = \xMax,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{SNR}$ (dB)},
ymode=log,
ymin=0.001,
ymax = \yMax=1,
yticklabels={{$\text{10}^{\text{-4}}$},{$\text{10}^{\text{-3}}$},{$\text{10}^{\text{-2}}$},{$\text{10}^{\text{-1}}$},{$\text{10}^{\text{0}}$}},
xticklabels={$\text{12}$,$\text{14}$,$\text{16}$,$\text{18}$,$\text{20}$,$\text{22}$,$\text{24}$},
yminorticks=true,
ylabel style={font=\color{white!15!black}},
%ylabel={SER},
axis background/.style={fill=white},
title style={font=\bfseries},
%title={16-QAM SER N = 1.024k,  $\Delta{p}$ = 1000 kHz},
xmajorgrids,
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
grid style={dotted,white!70!black}
]
\pgfplotsset{cycle list name=list1}
%+++++++++++ AWGN+++++++++++ 
\addplot %[color=ML_Demod, line width=1.0pt, mark=*]
  table[row sep=crcr]{%
12	0.203999794006348\\
13	0.129312927246094\\
14	0.0725995941162109\\
15	0.0351876449584961\\
16	0.0142747344970703\\
17	0.00464553070068359\\
18	0.0011612548828125\\
19	0.000215400695800781\\
20	3.66744995117188e-05\\
21	1.60446166992188e-05\\
22	1.45034790039063e-05\\
};

%+++++++++++ MCMA+++++++++++ 
\addplot %[color=Mcma, line width=1.0pt]
  table[row sep=crcr]{%
12	0.391968840297393\\
13	0.306107991623649\\
14	0.230668143891432\\
15	0.168168249407487\\
16	0.119854371611311\\
17	0.0848340070127593\\
18	0.0606591669101652\\
19	0.0444508376351417\\
20	0.033715293334632\\
21	0.0265755007954287\\
22	0.0217393104119996\\
};

%+++++++++++ UDDLMS+++++++++++ 
% \addplot %[color=LS, line width=1.0pt]
%   table[row sep=crcr]{%
% 12	0.429521776890361\\
% 13	0.270835987467939\\
% 14	0.146883972922957\\
% 15	0.0697918817570858\\
% 16	0.0298411171715204\\
% 17	0.0112029804227135\\
% 18	0.0036831596376741\\
% 19	0.00100522710301614\\
% 20	0.000228361092172333\\
% 21	4.23362877828642e-05\\
% 22	7.05334242394727e-06\\
% };

%+++++++++++ Louchet+++++++++++ 
\addplot %[color=LS_DDLMS, line width=1.0pt]
  table[row sep=crcr]{%
12	0.364393980714912\\
13	0.262124176163112\\
14	0.176297677023473\\
15	0.113027669556183\\
16	0.0688472452193111\\
17	0.0413365475146911\\
18	0.0248860832440505\\
19	0.0154395474172916\\
20	0.0102473377487744\\
21	0.00678153306710821\\
22	0.00489939450017856\\
};

%+++++++++++ Czegledi+++++++++++ 
\addplot %[color=LS_Czegledi, line width=1.0pt]
  table[row sep=crcr]{%
12	0.294615044966072\\
13	0.192365410213954\\
14	0.11564026330314\\
15	0.0628165887471186\\
16	0.0305152430115905\\
17	0.0131026508879582\\
18	0.00498658322781728\\
19	0.00170010713937859\\
20	0.000528846466023831\\
21	0.000158184799194832\\
22	4.65406967306256e-05\\
};

%+++++++++++ SW-Kabsch+++++++++++ 
\addplot %[color=LS_SW_Kabsch, line width=1.0pt]
  table[row sep=crcr]{%
12	0.255571921366189\\
13	0.16429575338463\\
14	0.0948819681179182\\
15	0.0491095905977079\\
16	0.0225148452972306\\
17	0.00895018018895491\\
18	0.0030423038213045\\
19	0.000888972760624655\\
20	0.000221510665238142\\
21	4.86591344436869e-05\\
22	9.88604266095256e-06\\
};
\end{axis}
\begin{axis}[%
width=\w cm,
height=\h cm,
at={(0cm,0cm)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax = \yMax,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}

\node at (0.5*\w,1*\h){\textbf{(a)}};
\node at (\w+1+0.5*\w,1*\h){\textbf{(b)}};
\node at (2*\w+2+0.5*\w,1*\h){\textbf{(c)}};


% \node at (0.5*\w,.85*\h)[font=\small]{$\Delta_p\cdot T = 10^{-8}$};
% \draw [black,very thick](0.18*\w,0.92*\h) rectangle (0.82*\w,.78*\h);

% \node at (\w+1+0.5*\w,.85*\h)[font=\small]{$\Delta_p\cdot T = 3.57\cdot 10^{-6}$};
% \draw [black,very thick](\w+1+0.18*\w,0.92*\h) rectangle  (\w+1+0.82*\w,.78*\h);

% \node at (2*\w+2+0.5*\w,.85*\h)[font=\small]{$\Delta_p\cdot T = 3.57\cdot 10^{-5}$};
% \draw [black,very thick](2*\w+2+0.18*\w,0.92*\h) rectangle (2*\w+2+0.82*\w,.78*\h);
\end{tikzpicture}%
